Invexifying Regularization of Non-Linear Least-Squares Problems

We consider regularization of non-convex optimization problems involving a non-linear least-squares objective. By adding an auxiliary set of variables, we introduce a novel regularization framework whose corresponding objective function is not only provably invex, but it also satisfies the highly desirable Polyak--Lojasiewicz inequality for any choice of the regularization parameter. Although our novel framework is entirely different from the classical $\ell_2$-regularization, an interesting connection is established for the special case of under-determined linear least-squares. In particular, we show that gradient descent applied to our novel regularized formulation converges to the same solution as the linear ridge-regression problem. Numerical experiments corroborate our theoretical results and demonstrate the method's performance in practical situations as compared to the typical $\ell_2$-regularization.

==> formatting/newcommands.tex <==
\makeatletter
\newcommand*{\transpose}{{\mathpalette\@transpose{}}}
\newcommand*{\@transpose}[2]{\raisebox{\depth}{$\m@th#1\intercal$}}

\newcommand{\hf}{\frac{1}{2}}

\newcommand{\fred}[1]{{\leavevmode\color{red}{Fred:\ #1}}}

%%%%%%%%%%%%%%%%%%%%%
% ---- vectors ---- %

\newcommand{\zero}{{\bf 0}}
\newcommand{\bfa}{{\bf a}}
\newcommand{\bfb}{{\bf b}}
\newcommand{\bfc}{{\bf c}}
\newcommand{\bfd}{{\bf d}}
\newcommand{\bfe}{{\bf e}}
\newcommand{\bff}{{\bf f}}
\newcommand{\bfg}{{\bf g}}
\newcommand{\bfh}{{\bf h}}
\newcommand{\bfi}{{\bf i}}
\newcommand{\bfj}{{\bf j}}
\newcommand{\bfk}{{\bf k}}
\newcommand{\bfl}{{\bf l}}
\newcommand{\bfm}{{\bf m}}
\newcommand{\bfn}{{\bf n}}
\newcommand{\bfo}{{\bf o}}
\newcommand{\bfp}{{\bf p}}
\newcommand{\bfq}{{\bf q}}
\newcommand{\bfr}{{\bf r}}
\newcommand{\bfs}{{\bf s}}
\newcommand{\bft}{{\bf t}}
\newcommand{\bfu}{{\bf u}}
\newcommand{\bfv}{{\bf v}}
\newcommand{\bfw}{{\bf w}}
\newcommand{\bfx}{{\bf x}}
\newcommand{\bfy}{{\bf y}}
\newcommand{\bfz}{{\bf z}}

%%%%%%%%%%%%%%%%%%%%%%
% ---- matrices ---- %

\newcommand{\bfA}{{\bf A}}
\newcommand{\bfB}{{\bf B}}
\newcommand{\bfC}{{\bf C}}
\newcommand{\bfD}{{\bf D}}
\newcommand{\bfE}{{\bf E}}
\newcommand{\bfF}{{\bf F}}
\newcommand{\bfG}{{\bf G}}
\newcommand{\bfH}{{\bf H}}
\newcommand{\bfI}{{\bf I}}
\newcommand{\bfJ}{{\bf J}}
\newcommand{\bfK}{{\bf K}}
\newcommand{\bfL}{{\bf L}}
\newcommand{\bfM}{{\bf M}}
\newcommand{\bfN}{{\bf N}}
\newcommand{\bfO}{{\bf O}}
\newcommand{\bfP}{{\bf P}}
\newcommand{\bfQ}{{\bf Q}}
\newcommand{\bfR}{{\bf R}}
\newcommand{\bfS}{{\bf S}}
\newcommand{\bfT}{{\bf T}}
\newcommand{\bfU}{{\bf U}}
\newcommand{\bfV}{{\bf V}}
\newcommand{\bfW}{{\bf W}}
\newcommand{\bfX}{{\bf X}}
\newcommand{\bfY}{{\bf Y}}
\newcommand{\bfZ}{{\bf Z}}

%%%%%%%%%%%%%%%%%%%%%%
% ---- iterates ---- %

\newcommand{\po}{\bfp_{0}}
\newcommand{\pt}{\bfp_{t}}
\newcommand{\ptt}{\bfp_{t+1}}

\newcommand{\xo}{\bfx_{0}}
\newcommand{\xt}{\bfx_{t}}
\newcommand{\xtt}{\bfx_{t+1}}

\newcommand{\fx}{f(\bfx)}
\newcommand{\fy}{f(\bfy)}
\newcommand{\fxo}{f(\xo)}
\newcommand{\fxt}{f(\xt)}
\newcommand{\fxtt}{f(\xtt)}

\newcommand{\gx}{\bfg(\bfx)}
\newcommand{\gy}{\bfg(\bfy)}
\newcommand{\gxo}{\bfg(\xo)}
\newcommand{\gxt}{\bfg(\xt)}
\newcommand{\gxtt}{\bfg(\xtt)}

\newcommand{\Jg}{\bfJ_{\bfg}}
\newcommand{\Jgx}{\Jg(\bfx)}
\newcommand{\Jgy}{\Jg(\bfy)}
\newcommand{\Jgxo}{\Jg(\xo)}
\newcommand{\Jgxt}{\Jg(\xt)}
\newcommand{\Jgxtt}{\Jg(\xtt)}

\newcommand{\Jtg}{\Jg^{\transpose}}
\newcommand{\Jtgx}{\Jtg(\bfx)}
\newcommand{\Jtgxo}{\Jtg(\xo)}
\newcommand{\Jtgxt}{\Jtg(\xt)}
\newcommand{\Jtgxtt}{\Jtg(\xtt)}

\newcommand{\fh}{\hat{f}}
\newcommand{\fhxp}{\fh(\bfx,\bfp)}
\newcommand{\fhyq}{\fh(\bfy,\bfq)}
\newcommand{\fhxpo}{\fh(\xo,\po)}
\newcommand{\fhxpt}{\fh(\xt,\pt)}
\newcommand{\fhxptt}{\fh(\xtt,\ptt)}

\newcommand{\etaxpyq}{{\bf \eta}(\bfx,\bfp,\bfy,\bfq)}

%%%%%%%%%%%%%%%%%%
% ---- sets ---- %

\newcommand{\sB}{\mathcal{B}}
\newcommand{\sD}{\mathcal{D}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\Rd}{\real^{d}}
\newcommand{\Rn}{\real^{n}}
\newcommand{\Rnd}{\real^{n \times d}}
